Capabilities of a fibered imager on an extremely large telescope

FIRST, the Fibered Imager foR a Single Telescope instrument, is an ultra-high angular resolution spectro-imager, able to deliver calibrated images and measurements beyond the telescope diffraction limit, a regime that is out of reach for conventional AO imaging. FIRST achieves sensitivity and accuracy by coupling the full telescope to an array of single mode fibers. Interferometric fringes are spectrally dispersed and imaged on an EMCCD. An 18-Fiber FIRST setup is currently installed on the Subaru Coronographic Extreme Adaptive Optics instrument at Subaru telescope. It is being exploited for binary star system study. In the late 2020 it will be upgraded with delay lines and an active LiNb03 photonic beam-combining chip allowing phase modulation to nanometer accuracy at MHz. On-sky results at Subaru Telescope have demonstrated that, thanks to the ExAO system stabilizing the visible light wavefront, FIRST can acquire long exposure and operate on significantly fainter sources than previously possible. A similar approach on a larger telescope would therefore offer unique scientific opportunities for galactic (stellar physics, close companions) and extragalactic observations at ultra-high angular resolution. We also discuss potential design variations for nulling and high contrast imaging.

==> FIRST - AO4ELT6(1)/1-Intro_first.tex <==
\section{INTRODUCTION}
\label{sec:intro}  % \label{} allows reference to this section

One of the key challenges in astronomy is the detection and characterization of faint companions such as exoplanets close to their host star. Achieving this requires both high performances in terms of angular resolution and dynamic range. Even though very large telescopes (8-meter class) were built and Extremely Large Telescopes (ELTs, 30-meter class) are on the horizon, reaching the desired performances is quite challenging especially for those ground based telescopes subject to turbulent atmosphere. 

To reach the diffraction limit of a telescope, several techniques were developed. Among them, the Adaptive Optics (AO) technique~\cite{rousset1990first} consists in using a deformable mirror to correct for the turbulence-induce aberrations on the incoming wavefront, allowing to restore the diffraction limit. However, because this correction is not perfect, residual speckle noise still limits the achievable dynamic range.

Other techniques were investigated. Speckle interferometry~\cite{labeyrie1970attainment} , based on the post processing of short exposure images, also allows to reach the diffraction limit of the telescope but still limits the dynamic range to a few 100. Aperture masking consists in placing a non-redundant mask in the pupil of the telescope and recombine the coherent light from each sub-aperture. This allows to retrieve spatial information at the highest spatial frequency of the telescope with contrast ratios down to $10^{-3}$~\cite{lacour2011sparse} . However it necessitate to sacrifice a large percentage of the full pupil because of the need of non-redundancy for the mask. In addition, speckle noise remains across each sub-aperture.

The method that can overcome the limitations of the aperture masking technique is the pupil remapping combined with the use of single-mode fibers\cite{perrin2006high} . On one hand, the pupil remapping allows one to use the whole aperture. On the other hand, the spatial filtering offered by the single-mode fibers allows to completely remove speckle noise over each sub-aperture. An instrument with such features is called FIRST (Fibered Imager foR a Single Telescope) and is currently installed on the 8-meter Subaru Telescope as part of the Subaru Coronographic Extreme Adaptive Optics~\cite{2015PASP..127..890J} (SCExAO) instrument. During its early development, FIRST revealed its power on the 3-meters Lick observatory performing spectroscopy analysis of the Capella binary system at the diffraction limit~\cite{huby2012first,huby2013first} . In this paper we present the integration and principle of FIRST as a module of SCExAO. We then present new upgrades for a version 2 (FIRST v2) of the instrument. Finally we discuss the interest of implementing FIRST, and more generally the interest of photonics instrument, on an ELT. 


==> FIRST - AO4ELT6(1)/2-First_v1.tex <==
\section{FIRST: pupil-remapping interferometry at the Subaru Telescope}

\subsection{FIRST, a module on SCExAO}
SCExAO is an instrument that is located on the Infra-Red (IR) Nasmyth platform of the Subaru telescope (see Fig.~\ref{fig:scexao_irnas}). It is fed by AO188~\cite{minowa2010performance}, a 188-element Curvature sensor adaptive optic system that delivers a first stage of wavefront correction. SCExAO main wavefront sensor is a pyramid wavefront sensor (PyWFS) in the visible (around $850$nm - see \textit{Lozi et al.}~\cite{Lozi_2019} for more details) delivering a wavefront quality over 80\% Strehl (in H-band), critical for high contrast imaging. SCExAO hosts a lot of different modules, and is divided over two benches: an IR and a Visible (Vis) bench. A dichroic filter on the IR bench and sends light (wavelengths $<900$nm) on the Vis bench through a periscope (see Fig.~\ref{fig:scexao_irnas}, right).

\begin{figure}[!h]
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.47\linewidth]{Figures/FIRST_SCEXAO.PNG} & \includegraphics[width=0.47\linewidth]{Figures/scexao_optics_first_visonly.PNG} \\
    \end{tabular}{}
    \caption{Left: SCExAO on the Infra-Red (IR) Nasmyth platfrom sits after AO188. SCExAO is composed of two benches on the top of the other, plus the FIRST recombination bench. SCExAO delivers light to CHARIS~\cite{Currie_2018} and MEC~\cite{walter2018mec} detectors. Right: A schematic of the optic path in the Visible bench and in the FIRST recombination bench.}
    \label{fig:scexao_irnas}
\end{figure}{}

The PyWFS usually operates between $850$ and $950$nm thanks to a pickoff filter wheel. Then the light can be split between VAMPIRES~\cite{norris2015vampires} and FIRST using a set of different filters on a filter wheel. All the light after the pyramid pickoff can also be sent either to FIRST with a mirror, or to VAMPIRES with an open slot.

\newpage
\subsection{Principle and setup}
FIRST combines the two techniques of pupil remapping and spatial filtering with single-mode fibers. Fig.~\ref{fig:firstv1_ppe} shows the principle of the instrument. The pupil of the telescope is divided into 18 different single mode fibers. The input pupil, redundant, is injected in the single-mode fibers with a 2D micro-lens array. The optimization of the injection is performed by an Iris AO segmented MEMS. Each segment is conjugated with a micro-lens (see Fig.~\ref{fig:firstv1_ppe2}a.) which focuses the beam into a single-mode fiber. A fiber bundle contains in total 36 single-mode fibers, that are then each connected at the other end to extension fibers that run to the recombination bench (see Fig.~\ref{fig:scexao_irnas}). On the recombination bench, the extension fibers are connected to single-mode fibers that end in a V-groove. The 18 used fibers form two sets of 9 fibers. The output of the two sets is 2 one-dimensional non redundant arrays each formed in a V-groove. Therefore, for each set of fibers, the N redundant baseline from the input pupil are now N non-redundant baselines corresponding to $N(N-1)/2$ different spatial frequencies. The outputs of each fibers are collimated (see Fig.~\ref{fig:firstv1_ppe2}b.) then recombined and spectrally dispersed with an equilateral SF2-prism. In order to increase the spectral resolution, an afocal anamorphic system, consisting in cylindrical lenses, stretches the beam in the dispersion direction and compresses it in the orthogonal direction. As shown on Fig~\ref{fig:firstv1_ppe2}c. the acquired fringe pattern contains information in terms of Optical Path Difference (OPD, phase, $\delta$) and in terms of spectrum (wavelength, $\lambda$). The spectral resolution obtained is empirically around $300$ @$700$nm.

\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{Figures/FIRST_ppe.PNG}
    \caption{Schematic diagram~\cite{kotani2009pupil} showing the principle of the FIRST instrument at the Subaru Telescope. The pupil of the Subaru Telescope is divided into several single-mode fibers thanks to a 2D micro-lens array. Light from the different fibers are then set into a one-dimensional non-redundant array, recombined and spectrally dispersed.  }
    \label{fig:firstv1_ppe}
\end{figure}{}

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.7\linewidth]{Figures/FIRST_ppe_2.PNG}
    \caption{a. Image of the micro-lens array conjugated with the Iris AO MEMs. b. One-dimesion non-redundant array: output of the V-groove from one set of 9 fibers. c. Recombination of one set of 9 fibers spectrally dispersed.}
    \label{fig:firstv1_ppe2}
\end{figure}{}

\subsection{Data reduction}\label{firstv1:data}

Typical FIRST images are two sets of fringes (one is shown on Fig~\ref{fig:firstv1_ppe2}c). The two sets are reduced separately, but rely on the same fringe analysis technique. After substraction of the dark, wavelength calibration and data curvature (caused by our optics) correction, we do a fringe fitting in the focal plane using the P2VM~\cite{millour2004data} method in each wavelength channel (each column of the image). This allows to compute closure phases for different baselines combinations. One nice feature of the closure phase measurement is that it allows to cancel differential phase errors between sub-apertures that can remain even after single-mode fiber filtering, Fitting a model of closure phase on the estimated closure phases allows to access spatial information about the observed object below the diffraction limit of the telescope. 
A new user-friendly data reduction pipeline is currently under development and should be completed by the beginning of 2020 to broaden the number of FIRST users.


\subsection{Science with FIRST}
Typical targets of interest for FIRST are close binary systems or surface of large resolved stars. An ultimate goal for this concept would be the direct detection and characterization of an exoplanet.
At the Subaru Telescope, FIRST already showed that it could detect a companion below the diffraction limit (18 mas @700nm). Indeed, on the Alpha Equ binary system, a companion was detected with at a separation of around 10mas, or almost half of the telescope diffraction limit. These data are still under analysis.



==> FIRST - AO4ELT6(1)/3-First_v2.tex <==
\section{FIRSTv2: photonics upgrades}

While FIRST can still take data on-sky, upgrades are in preparation. One of the advantages to have two sets of 9 fibers is that one of them can be upgraded while the other is still in use. Fig.~\ref{fig:firstv2_ppe} shows the schematic diagram of FIRST v2, with three major upgrades.

\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{Figures/FIRSTv2_ppe.PNG}
    \caption{Schematic diagram showing the principle of FIRSTv2. Upgrades compared to FIRSTv1 are the fiber delay lines, the electro-optic photonic phase controller-recombiner and the camera.}
    \label{fig:firstv2_ppe}
\end{figure}{}


\subsection{Fiber path length matching}
Current single-mode fiber extensions on FIRST were all manufactured together and then polished by hand to match the path length. If/whenever one breaks it is then time consuming and complicated to make a new one and match the path length with the others. To prevent this, and to have a better accuracy on the path length matching of the current fibers, we want to implement fiber delay lines (see Fig.~\ref{fig:Delay_lines}) between the fibers from the fiber bundle and the extension fibers.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{Figures/delay_line.PNG}
    \caption{Left: Optical path inside the delay line. The input beam reflects on a movable mirror and is then re-injected in the output fiber. Right: Picture of a delay line.}
    \label{fig:Delay_lines}
\end{figure}{}

Fig.~\ref{fig:Delay_lines} shows on the left the optic path inside the delay line. The light from the input fiber is collimated, bounces on two movable mirrors and is then re-injected in the output fiber. The mirrors sit on a lead screw that is linked to a motor. The total OPD range is of $100mm$, the OPD resolution is $0.4134\mu m$ and the OPD accuracy is $1$ to $2\mu m$. 

\subsection{Active photonic chip}
The second upgrade is the integration of an integrated optic active chip. Fig.~\ref{fig:firstv2_iochip} shows the three different components of this chip:
\begin{itemize}
    \item \textbf{A: The silica Y-junction splitters} split each of the 9 input waveguides in 8. Meaning there are 9 inputs and 72 outputs.
    \item \textbf{B: The Lithium Niobate chip} takes in the 72 straight waveguides. As shown Fig.~\ref{fig:firstv2_iochip} a potential difference can be applied across the waveguides. The consequence of this is a change of the Lithium Niobate refractive index, modifying the phase in the waveguides. This allows to control the phase delay inside each waveguide at high speed (MHz).
    \item \textbf{C: The Silica beam-combining chip} takes in the 72 waveguides and recombines them two by two. Doing so, we have 36 outputs that are the 36 different baselines (similar to current FIRST version). The difference here is that instead of being all superimposed, the lights from each baseline are well separated at the output of the combining chip. A phase ramp is then applied to obtain the OPD information.
\end{itemize}{}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{Figures/io_chip.PNG}
    \caption{New integrated optic active chip composed by 3 elements: the Silica Y-junctions that split each input, the Lithium Niobate chip that allows a phase control within each waveguides and the Silica beam-combining chip to form recombine the different pairs.}
    \label{fig:firstv2_iochip}
\end{figure}{}


\subsection{New output data}
As mentioned in Section~\ref{firstv1:data}, the current data in FIRST is the superimposition of all the interference patterns between the different baselines, spectrally dispersed. Each image then contains spectral and OPD information. With FIRST v2, the output data is little different. A typical image on the camera of the output of the beam-combining chip after spectral dispersion is shown on Fig.~\ref{fig:firstv2_cam}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.4\linewidth]{Figures/camera.PNG}
    \caption{Data output for FIRST v2. Each of the 36 outputs of the beam-combining chip are dispersed with a prism, and are all separated.}
    \label{fig:firstv2_cam}
\end{figure}{}

In this case, one image only gives a spectral information and an intensity. To retrieve the OPD information, one needs to modulate the phase in each waveguide and record series of images: the fringes are temporally encoded. To do so a voltage ramp is applied on the chip B (Fig.~\ref{fig:firstv2_iochip}) to temporally scan the OPD For the data reduction, a similar fringe fitting using the V2PM method is used.


All these upgrades will be brought to the Subaru Telescope in late 2020 or early 2021, and could potentially increase the stability and sensitivity of the instrument.

==> FIRST - AO4ELT6(1)/4-Capabilities_ELT.tex <==
\section{Capabilities of a photonic imager on an Extremely Large Telescope}

We saw how the FIRST instrument concept could be powerful on an 8m telescope like Subaru, enabling detection and spectroscopy below the limit of the telescope. When the concept was born, it was already envisioned~\cite{perrin2006high} for 30-meter class telescopes. We would like to bring forward again this vision at the end of this paper, presenting different use of FIRST on a segmented ELT and trying to estimate the performance that could be expected.

\subsection{FIRST-like instrument on an ELT}
The spatial resolution of a 30-meter class telescope is around $5$mas @$700$nm. According to our experience at the Subaru Telescope, we saw that FIRST was able to detect a companion at roughly half of the diffraction limit. This would mean that FIRST on a 30-meter class telescope could potentially be able to detect and characterize companions at around $2.5$mas from the host star. 

In terms of achievable contrast \textit{B. Norris and al.}~\cite{norris2014high} showed that in the case of a pupil-remapping interferometer, the contrast ratio detection at $1\sigma$ was directly proportional to the on-sky closure-phase stability. The latest not only relies on the stability of the instrument itself, but also on the stability of the adaptive optics system. Since an high contrast imager on an ELT would most likely have an extreme adaptive optics system, it is easy to infer that the ExAO-corrected phase error would be a few dozens of nm. The stability of the closure phase in-lab is around $0.01\deg$ from experience. We can then estimate thanks to \textit{B. Norris and al.}~\cite{norris2014high} equations (4) and (5) that the achievable contrast of FIRST on an ELT would be of the order of $10^{-6}$. 

Finally, the sensitivity of the instrument scales with the amount of light injected in the single-mode fibers hence the size of the sub-aperture. Fig.~\ref{fig:first_elt} shows two different setups that can be imagined for FIRST on an ELT. If only one or seven segments per sub-aperture are shown here, in practice we would want more sub-apertures per fiber to maximize the sensitivity. Another way to increase the sensitivity of the instrument would be to use an MKIDS~\cite{walter2018mec} detector or on-chip MKIDS-like detector~\cite{cheng2019broadband} allowing to have a spectrometer directly on the chip with no read-out-noise.
%If the size of the sub-aperture was 1 segment, it would be quite similar to the size of the sub-apertures at the Subaru Telescope where we empirically found that the magnitude limit of our instrument was around $6.5$. In similar conditions, we can say that it would be the same for a configuration with one segment on an ELT. An extrapolation allows us to estimate that if the sub-apertures were composed by 7 segments, the magnitude limit would be around $11.5$.

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.45\linewidth]{Figures/FIRST_elt.PNG}
    \caption{FIRST concept on a large multi-aperture telescope
(small portion of the segmented mirror shown here). Light from different amount of segments can be injected in a single-mode fiber, changing the sensitivity of the instrument. The light from the fibers could then go through an integrated optics active chip, whose output could be imaged on a read-out-noise-free MKIDS detector.}
    \label{fig:first_elt}
\end{figure}{}

\subsection{Other possibilities with photonics}
An often overlooked benefit of the ELT generation is that the huge telescope diameter brings single-aperture interferometric techniques (FIRST, GLINT~\cite{lagadec2018glint} , aperture masking) closer to the realm of long-baseline interferometry (GRAVITY~\cite{eisenhauer2007gravity} , OHANA~\cite{perrin2000fibered}). In fact, many techniques and technologies developed for long-baseline interferometry can be directly applied to ELTs, with minimal modification (as we discussed in the previous section in the particular case of FIRST).

More interestingly, ELTs bring a hybrid space perfect for new technologies. One such technology is on-chip kernel nulling~\cite{martinache2018kernel,goldsmith2017improving} . In this concept (see Fig.~\ref{fig:kernel}), photonic circuitry consisting of cascaded multimode interference couplers (MMIs) interferes the light in a particular way to not only null the starlight (destructively interfere on-axis starlight that causes photon noise), but additionally interfere the light in a particular way such that the resulting flux outputs form Kernel observables. These Kernels have the same properties as closure phase, and are extremely robust against second order phase error from the atmosphere. They also are a way to increase the achievable contrast compared to previous section. A simple analogy would be to combine the detection contrasts of a coronagraph with the astrometry precision of GRAVITY and the spectral capability of IRD~\cite{kotani2018infrared} . 

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/kernel.PNG}
    \caption{Left: Beam propagation simulation of a MultiMode interference coupler (MMI) corresponding to the $4\times 4$ MMI
    (\textbf{N}). The four input beams are interfered such that all starlight is sent to the bright output port. Right: The Kernel-nuller
    concept composed of $2$ MMIs separated by modulated phase shifters used to eliminate background fluctuations. The $3$ 'dark' ports
    feed the kernel-scrambler (\textbf{S}) matrix which produces the kernel-null observables. }
    \label{fig:kernel}
\end{figure}{}
